XMM-Newton Resolves Parsec-scale X-ray Jets in the PeVatron Microquasar V4641 Sgr

The microquasar V4641 Sagittarii (V4641 Sgr) has recently been established as one of the most powerful Galactic PeV cosmic-ray accelerators (PeVatrons) through the detection of degree-scale gamma-ray emission to 0.8 PeV. Using XMM-Newton, we performed an X-ray survey of its gamma-ray-emitting regions during the quiescent phase. We discovered extended X-ray emission to the north and south of V4641 Sgr, aligned with the radio-jet axis, revealing X-ray jet structures extending over several tens of parsecs for the first time. The northern and southern knot-like features, dubbed n1 and s1, are located approximately 20 pc from the central binary and spatially coincident with the gamma-ray emission. The X-ray emission from each knot, characterized by a photon index of $\Gamma_X = 1.9 \pm 0.1_{\rm stat} \pm 0.5_{\rm syst}$ and an energy flux of $\sim$(2--4)$\times10^{-13}$~erg~cm$^{-2}$~s$^{-1}$ in the 2--10 keV band, is likely non-thermal in origin, indicating synchrotron radiation from accelerated electrons. The morphological coincidence between the X-ray and gamma-ray emission favors a leptonic scenario for the gamma rays, although the X-ray emission is more compact than the gamma-ray-emitting region and the hadronic scenario cannot be excluded. Through X-ray to gamma-ray modeling, we obtain a weak magnetic field strength of 3--5~$\mu$G. We propose that the newly detected X-ray knots represent particle-acceleration sites, such as jet termination or (re-)collimation regions powered by V4641 Sgr, or downstream structures analogous to the knots of the outer jets in SS~433/W50. This discovery suggests that extended X-ray emission along jets would be a key signature, yet previously overlooked, in PeVatron microquasars.

==> table1.tex <==

\begin{table}[]
    \begin{center}
    \caption{
%    \nt{to be updated.}
    Spatial and spectral information of X-ray knots.
    \label{tab:fit} }
    %
    \begin{tabular}{c | c | c | c | c }
    \hline \hline 
         & n1 & s1 & w1 & s2 \\
    \hline
    R.A. (deg)     & 274.834     & 274.881   & 274.736  & 274.689 \\
    Decl. (deg)    & $-$25.207   & $-$25.631 & $-$25.444 & $-$26.111 \\
    $\sigma_{\rm major}$ (arcmin) & 3.4 $\pm$ 0.3 & 2.6 $\pm$ 0.4 & 3.5 $\pm$ 0.2 & 4.4 $\pm$ 0.6 \\ 
    $\sigma_{\rm minor}$ (arcmin) & 2.0 $\pm$ 0.2 & 2.3 $\pm$ 0.3 & 2.8 $\pm$ 0.2 & 3.8 $\pm$ 0.3  \\ 
    Angle (deg)   &  13 $\pm$ 0.1 & $-0.3 \pm 0.6$  & $-35$ $\pm$ 0.2 & 67 $\pm$ 0.2 \\ 
    Distance from \src\ (arcmin)  &  12 & 14  & 6.4 & 43  \\
    Distance from \src\ (pc)$^{\rm (a)}$ &  23 & 25 & 12 & 78 \\
    \hline 
    \NH\ ($10^{21}$~\column) & $1.7 \pm 0.4$    & 1.7 (fixed) & 1.7 (fixed) & 1.7 (fixed)  \\
    $\Gamma$                 & $1.9 \pm 0.1$ &  $1.9 \pm 0.2$ & 2 (fixed) & 2 (fixed) \\
    $F_{\rm 2-10~keV}$ ($10^{-13}$~\eflux) &  $2.1 \pm 0.2 $ & $2.7 \pm 0.4$ & $<0.40$ & $<2.2$ \\
    $SB_{\rm 2-10~keV}$ ($10^{-15}$~\eflux~arcmin$^{-2}$) &  $7.4 \pm 0.7$  & $5.1 \pm 0.8$  & $<2.6 $  & $<5.3$ \\
    $\chi^2$ (dof) & & &   \\
    \hline
    \end{tabular}
    \end{center}
\tablecomments{
\nt{should remove w1 and s2 as they are marginal detection?}
\nt{these numbers may be subject to change.}
\\
Coordinates, major and minor axes, and position angle (counterclockwise to the north) are obtained by the 2--4.5 keV image shown in Figure~\ref{fig:diffuse}. \\
Only statistical uncertainty is shown, while there is $\sim30$\% systematic uncertainty on the photon index and flux. \\
The upper limit was derived at $2\sigma$ c.l. \\
$^{\rm (a)}$ $d=6.2$~kpc is assumed.
}
\end{table}



\begin{table}[]
    \centering
    \caption{
    \nt{to be updated.}
    Spatial and spectral information of X-ray knots.
    \label{tab:fit} }
    %
    \begin{tabular}{c | cc | c | c | c }
    \hline \hline 
         & \multicolumn{2}{c|}{n1} & s1 & w1 & s2 \\
    \hline
    R.A. (deg)     & \multicolumn{2}{c |}{274.834}     & 274.881   & 274.736  & 274.689 \\
    Decl. (deg)    & \multicolumn{2}{c |}{$-$25.207}   & $-$25.631 & $-$25.444 & $-$26.111 \\
    $\sigma_{\rm major}$ (arcmin) & \multicolumn{2}{c|}{3.4 $\pm$ 0.3} & 2.6 $\pm$ 0.4 & 3.5 $\pm$ 0.2 & 4.4 $\pm$ 0.6 \\ 
    $\sigma_{\rm minor}$ (arcmin) & \multicolumn{2}{c|}{2.0 $\pm$ 0.2} & 2.3 $\pm$ 0.3 & 2.8 $\pm$ 0.2 & 3.8 $\pm$ 0.3  \\ 
    Angle (deg)   &  \multicolumn{2}{c|}{13 $\pm$ 0.1} & $-0.3 \pm 0.6$  & $-35$ $\pm$ 0.2 & 67 $\pm$ 0.2 \\ 
    Distance from \src\ (arcmin)  & \multicolumn{2}{c|}{ 12} & 14  & 6.4 & 43  \\
    Distance from \src\ (pc)$^{\rm (a)}$ &  \multicolumn{2}{c|}{23} & 25 & 12 & 78 \\
    \hline 
    \NH\ ($10^{21}$~\column) & $3.5 \pm 1.9$   & 2.3 (fixed) & 3.5 (fixed) \\
    $\Gamma$                 & $1.78 \pm 0.09$ & $1.79 \pm 0.09$ & $1.8 \pm 0.4$  \\
    $F_{\rm 2-10~keV}$ ($10^{-13}$~\eflux) &  & & 2.8 $\pm$ 0.1 \\
    $SB_{\rm 2-10~keV}$ ($10^{-15}$~\eflux~arcmin$^{-2}$) &  $9.6 \pm 0.8$ &   &  $6.7 \pm 0.2$\\
%    $\chi^2$/dof & & &  0.98/36 \\
    \hline
    \end{tabular}
\tablecomments{
Coordinates, major and minor axes, and position angle (counterclockwise to the north) are obtained by the 2--4.5 keV image shown in Figure~\ref{fig:diffuse}. \\
$^{\rm (a)}$ $d=6.2$~kpc is assumed.
}
\end{table}

